Gaussian Mixture Graphical Lasso with Application to Edge Detection in Brain Networks

Sparse inverse covariance estimation (i.e., edge de-tection) is an important research problem in recent years, wherethe goal is to discover the direct connections between a set ofnodes in a networked system based upon the observed nodeactivities. Existing works mainly focus on unimodal distributions,where it is usually assumed that the observed activities aregenerated from asingleGaussian distribution (i.e., one graph).However, this assumption is too strong for many real-worldapplications. In many real-world applications (e.g., brain net-works), the node activities usually exhibit much more complexpatterns that are difficult to be captured by one single Gaussiandistribution. In this work, we are inspired by Latent DirichletAllocation (LDA) [4] and consider modeling the edge detectionproblem as estimating a mixture ofmultipleGaussian distribu-tions, where each corresponds to a separate sub-network. Toaddress this problem, we propose a novel model called GaussianMixture Graphical Lasso (MGL). It learns the proportionsof signals generated by each mixture component and theirparameters iteratively via an EM framework. To obtain moreinterpretable networks, MGL imposes a special regularization,called Mutual Exclusivity Regularization (MER), to minimize theoverlap between different sub-networks. MER also addresses thecommon issues in read-world data sets,i.e., noisy observationsand small sample size. Through the extensive experiments onsynthetic and real brain data sets, the results demonstrate thatMGL can effectively discover multiple connectivity structuresfrom the observed node activities

==> table.tex <==
\begin{table*}[!ht]
    \centering 
    \caption{Important Notations.}\vspace{-5pt}\label{tab:notation}
    \begin{tabular}{|r|l|}
    \hline\vspace{-5pt}&\\
    Symbol& Definition\\
    \hline\vspace{-5pt}&\\
    $D$ & The number of variables or objects\\
    $N$ & The number of samples \\
    $K$ & The number of distribution \\
    $\mb{X}$ & The observations of $D$-variate Gaussian distribution \\
    $\mb{S}$ & The  empirical  covariance  matrix of $\mb{X}$ \\
    $\phi_k$ & The prior probability or mixing coefficient of distribution k \\
    $r_{ik}$ & The posterior probability of sample i generated from distribution k \\
    $\mb{\Sigma}_k$ & The covariance matrix of distribution k \\
    $\mb{\Theta}_k$ & The precision matrix of distribution k \\
    $\bar{\mb{\Theta}}_k$ & The non-negative copy of $\mb{\Theta}_k$ with zero diagonal elements\\
    $\lambda_1$ &  The Lagrangian multiplier of general lasso regularization\\ 
    $\lambda_2 $ &  The Lagrangian multiplier of mutual exclusivity regularization \\ 
        \hline
    \end{tabular}
    
\vspace{5pt}
\end{table*}
